Stochastic Neural Radiance Fields: Quantifying Uncertainty in Implicit 3D Representations

Neural Radiance Fields (NeRF) has become a popular framework for learning implicit 3D representations and addressing different tasks such as novel-view synthesis or depth-map estimation. However, in downstream applications where decisions need to be made based on automatic predictions, it is critical to leverage the confidence associated with the model estimations. Whereas uncertainty quantification is a long-standing problem in Machine Learning, it has been largely overlooked in the recent NeRF literature. In this context, we propose Stochastic Neural Radiance Fields (S-NeRF), a generalization of standard NeRF that learns a probability distribution over all the possible radiance fields modeling the scene. This distribution allows to quantify the uncertainty associated with the scene information provided by the model. S-NeRF optimization is posed as a Bayesian learning problem which is efficiently addressed using the Variational Inference framework. Exhaustive experiments over benchmark datasets demonstrate that S-NeRF is able to provide more reliable predictions and confidence values than generic approaches previously proposed for uncertainty estimation in other domains.

==> table_KL.tex <==
\begin{table}[t]
\centering
\resizebox{.5\textwidth}{!}{
\begin{tabular}{llccclccc}
\multicolumn{1}{c}{} &
   &
  \multicolumn{3}{c}{\textbf{Neg. Log. Likelihood(NLL) $\downarrow$}} &
   &
  \multicolumn{3}{c}{\textbf{MSE-Uncertainty Correlation $\uparrow$}} \\ \cline{3-5} \cline{7-9} 
\multicolumn{1}{c}{} &
   &
  \textbf{w/o KL} &
  \textbf{w/ KL} &
  \textbf{S-NeRF} &
   &
  \textbf{w/o KL} &
  \textbf{w/ KL} &
  \textbf{S-NeRF} \\ \cline{1-1} \cline{3-5} \cline{7-9} 
\cellcolor[HTML]{FFFFFF}\textbf{Flower} &
   &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1.41} &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 2.18} &
  \cellcolor[HTML]{FFFFFF}\textbf{1.27} &
   &
  \cellcolor[HTML]{FFFFFF}0.54 &
  \cellcolor[HTML]{FFFFFF}0.51 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.63} \\
\cellcolor[HTML]{FFFFFF}\textbf{Frotress} &
   &
  \cellcolor[HTML]{FFFFFF}1.26 &
  \cellcolor[HTML]{FFFFFF}0.82 &
  \cellcolor[HTML]{FFFFFF}\textbf{-0.03} &
   &
  \cellcolor[HTML]{FFFFFF}0.31 &
  \cellcolor[HTML]{FFFFFF}0.53 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.55} \\
\cellcolor[HTML]{FFFFFF}\textbf{Leaves} &
   &
  \cellcolor[HTML]{FFFFFF}0.98 &
  \cellcolor[HTML]{FFFFFF}0.96 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.68} &
   &
  \cellcolor[HTML]{FFFFFF}0.60 &
  \cellcolor[HTML]{FFFFFF}0.65 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.73} \\
\cellcolor[HTML]{FFFFFF}\textbf{Horns} &
   &
  \cellcolor[HTML]{FFFFFF}3.08 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.75} &
  \cellcolor[HTML]{FFFFFF}\textbf{0.60} &
   &
  \cellcolor[HTML]{FFFFFF}0.53 &
  \cellcolor[HTML]{FFFFFF}0.64 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.70} \\
\cellcolor[HTML]{FFFFFF}\textbf{Trex} &
   &
  \cellcolor[HTML]{FFFFFF}1.82 &
  \cellcolor[HTML]{FFFFFF}1.54 &
  \cellcolor[HTML]{FFFFFF}\textbf{1.37} &
   &
  \cellcolor[HTML]{FFFFFF}0.58 &
  \cellcolor[HTML]{FFFFFF}0.66 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.68} \\
\cellcolor[HTML]{FFFFFF}\textbf{Fern} &
   &
  \cellcolor[HTML]{FFFFFF}2.46 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{1.63}} &
  \cellcolor[HTML]{FFFFFF}2.01 &
   &
  \cellcolor[HTML]{FFFFFF}0.51 &
  \cellcolor[HTML]{FFFFFF}0.66 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.69} \\
\cellcolor[HTML]{FFFFFF}\textbf{Orchids} &
   &
  \cellcolor[HTML]{FFFFFF}4.45 &
  \cellcolor[HTML]{FFFFFF}2.37 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{1.95}} &
   &
  \cellcolor[HTML]{FFFFFF}0.31 &
  \cellcolor[HTML]{FFFFFF}0.59 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.65} \\
\cellcolor[HTML]{FFFFFF}\textbf{Room} &
   &
  \cellcolor[HTML]{FFFFFF}4.39 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 3.49} &
  \cellcolor[HTML]{FFFFFF}\textbf{2.35} &
   &
  \cellcolor[HTML]{FFFFFF}0.54 &
  \cellcolor[HTML]{FFFFFF}0.65 &
  \cellcolor[HTML]{FFFFFF}\textbf{0.74} \\ \cline{1-1} \cline{3-5} \cline{7-9}
\textbf{Avg.} &
   &
  2.48 &
  1.72 &
  \textbf{1.28} &
   &
  0.49 &
  0.61 &
  \textbf{0.67} \\
\end{tabular}}
\caption{\textbf{The effect of the prior constraints.} Conducting KL divergence constraints by a prior with high fixed variance (w/KL) dramatically improves the model's performance on NLL and MSE-Uncertainty correlation. An additional prior with optimizable variance over the training set further enhances the model's performance as well as stability.}
\label{tab:priorconstraints}
\vspace{-3mm}
\end{table}

==> table_results.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\multicolumn{1}{c}{} &
   &
  \multicolumn{4}{c}{\textbf{Neg. Log. Likelihood (NLL) $\downarrow$}} &
   &
  \multicolumn{4}{c}{\textbf{MSE-Uncertainty Correlation $\uparrow$}} \\ \cline{3-6} \cline{8-11} 
\multicolumn{1}{c}{} &
   &
  \textbf{MC-DO~\cite{mc-dropout}} &
  \textbf{D. Ens.~\cite{deepensemble}} &
  \textbf{NeRF-W~\cite{nerfwild}} &
  \textbf{S-NeRF} &
   &
  \textbf{MC-DO~\cite{mc-dropout}} &
  \textbf{D. Ens.~\cite{deepensemble}} &
  \textbf{NeRF-W~\cite{nerfwild}} &
  \textbf{S-NeRF} \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\textbf{Flower}   &  & 4.63 & 1.63 & 1.71 & \textbf{1.27}  &  & 0.38 & 0.59 & 0.49 & \textbf{0.63} \\
\textbf{Frotress} &  & 5.19 & 2.29 & 1.04 & \textbf{-0.03} &  & 0.24 & 0.37 & 0.44 & \textbf{0.55} \\
\textbf{Leaves}   &  & 2.72 & 2.66 & 0.79 & \textbf{0.68}  &  & 0.39 & 0.57 & 0.65 & \textbf{0.73} \\
\textbf{Horns}    &  & 4.18 & 2.17 & 0.78 & \textbf{0.60}  &  & 0.43 & 0.50 & 0.50 & \textbf{0.70} \\
\textbf{Trex}     &  & 4.10 & 2.28 & 1.91 & \textbf{1.37}  &  & 0.42 & 0.53 & 0.66 & \textbf{0.68} \\
\textbf{Fern}     &  & 4.90 & 2.47 & 2.16 & \textbf{2.01}  &  & 0.50 & 0.65 & 0.59 & \textbf{0.69} \\
\textbf{Orchids}  &  & 5.74 & 2.23 & 2.24 & \textbf{1.95}  &  & 0.50 & 0.60 & 0.60 & \textbf{0.65} \\
\textbf{Room} &
   &
  5.06 &
  {\color[HTML]{333333} \textbf{2.13}} &
  4.93 &
  2.35 &
   &
  0.46 &
  0.65 &
  0.38 &
  \textbf{0.74} \\ \cline{1-1} \cline{3-6} \cline{8-11} 
\textbf{Avg.}     &  & 4.57 & 2.23 & 1.95 & \textbf{1.27}  &  & 0.40 & 0.56 & 0.54 & \textbf{0.67}
\end{tabular}}
\vspace{1mm}
\caption{\textbf{Results for the uncertainty estimation metrics obtained by all the evaluated methods on the NeRF LLFF dataset~\cite{nerf}.}}
\label{tab:results}
\vspace{-5mm}
\end{table*}

==> table_time.tex <==
\begin{table}[t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c }
\hline
 &
  \textbf{MC-DO~\cite{mc-dropout}} &
  \textbf{D. Ens.~\cite{deepensemble}} &
  \textbf{NeRF-W~\cite{nerfwild}} &
  \textbf{S-NeRF} \\
  \hline
Inference (sec.) &
  \multicolumn{1}{r}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 38.26}} &
  \multicolumn{1}{r}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 34.77}} &
  \multicolumn{1}{r}{\cellcolor[HTML]{FFFFFF}7.08} &
  \multicolumn{1}{r}{\cellcolor[HTML]{FFFFFF}\textbf{6.06}}\\
  \hline
\end{tabular}}
\vspace{1mm}
\caption{\textbf{Rendering time} (s) required by the evaluated methods for a single view with resolution 500$\times$400.}
\vspace{-8mm}
\label{tab:time}
\end{table}

